LayerNAS: Neural Architecture Search in Polynomial Complexity

Neural Architecture Search (NAS) has become a popular method for discovering effective model architectures, especially for target hardware. As such, NAS methods that find optimal architectures under constraints are essential. In our paper, we propose LayerNAS to address the challenge of multi-objective NAS by transforming it into a combinatorial optimization problem, which effectively constrains the search complexity to be polynomial. For a model architecture with $L$ layers, we perform layerwise-search for each layer, selecting from a set of search options $\mathbb{S}$. LayerNAS groups model candidates based on one objective, such as model size or latency, and searches for the optimal model based on another objective, thereby splitting the cost and reward elements of the search. This approach limits the search complexity to $ O(H \cdot |\mathbb{S}| \cdot L) $, where $H$ is a constant set in LayerNAS. Our experiments show that LayerNAS is able to consistently discover superior models across a variety of search spaces in comparison to strong baselines, including search spaces derived from NATS-Bench, MobileNetV2 and MobileNetV3.

==> 00_abstract_copy.tex <==
 models discovered through LayerNAS achieve higher top-1 accuracy on ImageNet \blue{when compared to} both \blue{the} baseline models and \blue{the} models discovered by other NAS algorithms: \blue{we achieve} 69\% \blue{on} 61M MAdds, 75.6\% \blue{on} 229M MAdds, 77.1\% \blue{on} 322M MAdds, 78.3\% \blue{on} 622M MAdds. 


